Mitigating Saliency Collapse: Robust Saliency-Aware Long-Text Image-Text Alignment

Long-text image-text alignment is essential for fine-grained scene understanding, yet existing methods mainly focus on extending context length or improving local alignment. We identify an overlooked failure mode, saliency collapse, where models over-rely on text that features visual prominence while underutilizing non-salient context. Consequently, retrieval performance degrades sharply when salient content is reduced, despite that the non-salient context remains informative. To address this, we propose RoSA, a saliency-aware finetuning framework that decomposes image-text pairs into complementary salient and contextual views, enabling joint learning of prominent and contextual semantics. We propose a modality-independent decomposition strategy to combine object-level visual saliency estimation with LLM-based text decomposition to bridge vision and language. We employ auxiliary objectives to explicitly align these views, ensuring robust representation with both salient and contextual features. RoSA greatly improves long-text retrieval and demonstrates strong robustness to saliency collapse across benchmarks. Moreover, our auxiliary objectives are plug-and-play, bringing consistent gains to existing tuning methods. Code and checkpoints are available at: https://github.com/intelligolabs/RoSA.

==> section/preliminary_old.tex <==
\section{Preliminary study}\label{sec:preliminary}
\begin{table}[t]
\centering
\caption{
\textbf{Length-controlled diagnosis under progressive salient omission.}
Each cell reports the relative R@1 drop under salient deletion / matched random-span deletion, computed with respect to each model's original R@1.
The value below each $\alpha$ header is the fraction of removed caption tokens.
Across datasets and baselines, deleting salient phrases causes much larger degradation than deleting random contiguous spans of the same length.
}
\label{tab:preliminary_diagnosis}

\footnotesize
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.15}

\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}l ccc ccc ccc@{}}
\toprule
& \multicolumn{3}{c}{\textbf{DOCCI}}
& \multicolumn{3}{c}{\textbf{PathGen}}
& \multicolumn{3}{c}{\textbf{INSECT}} \\
\cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}
Model
& $\alpha\!=\!75$ & $\alpha\!=\!25$ & $\alpha\!=\!0$
& $\alpha\!=\!75$ & $\alpha\!=\!25$ & $\alpha\!=\!0$
& $\alpha\!=\!75$ & $\alpha\!=\!25$ & $\alpha\!=\!0$ \\
\textit{removed (\%)}
& \textcolor{mildblue}{5.67} & \textcolor{midorange}{33.70} & \textcolor{severered}{57.95}
& \textcolor{mildblue}{1.96} & \textcolor{midorange}{31.28} & \textcolor{severered}{67.30}
& \textcolor{mildblue}{6.45} & \textcolor{midorange}{34.31} & \textcolor{severered}{65.53} \\
\midrule
LongCLIP-FT
& 11.48/1.78 & 34.07/16.68 & 67.88/39.17
& 58.08/1.97 & 69.00/22.93 & 85.81/57.42
& 49.24/6.28 & 55.84/17.86 & 66.34/24.78 \\
GOAL
& \phantom{0}7.70/1.59 & 26.53/15.74 & 62.50/37.76
& 25.43/1.54 & 56.07/28.52 & 89.60/69.94
& 17.00/1.82 & 34.82/22.47 & 61.94/47.77 \\
StructXLIP
& 10.29/1.53 & 29.39/15.53 & 63.27/37.90
& 33.54/0.84 & 56.18/20.75 & 87.00/63.94
& 21.24/6.43 & 39.42/24.28 & 65.48/50.59 \\
\bottomrule
\end{tabular}%
}

\vspace{2pt}
{\scriptsize All numbers are percentages. \textit{removed (\%)} denotes the fraction of removed caption tokens. A negative random-span drop means matched random deletion slightly improves R@1.}
\end{table}
% \begin{table}[t]
% \centering
% \caption{
% \textbf{Salient-only diagnosis.}
% We feed each model only the top-$k\%$ most salient phrases of every caption, with all non-salient context removed.
% Cells report R@1 (\%) on text-to-image retrieval.
% The \textit{Full}$^\dagger$ column reports each model's R@1 using the original complete caption.
% The $k{=}100$ setting isolates the standalone contribution of all salient phrases, while smaller $k$ values measure how retrieval degrades when fewer salient phrases are available.
% The near-random performance at $k{=}0$ serves as a sanity check, since both salient and non-salient text are removed.
% }
% \label{tab:salient_only}

% \scriptsize
% \setlength{\tabcolsep}{2.2pt}
% \renewcommand{\arraystretch}{1.08}

% \resizebox{\linewidth}{!}{%
% \begin{tabular}{@{}l c|cccccc c|cccccc c|cccccc@{}}
% \toprule
% & \multicolumn{7}{c}{\textbf{DOCCI}}
% & \multicolumn{7}{c}{\textbf{PathGen}}
% & \multicolumn{7}{c}{\textbf{INSECT}} \\
% \cmidrule(lr){2-8}\cmidrule(lr){9-15}\cmidrule(lr){16-22}
% Model
% & \textit{Full}$^\dagger$ & 100 & 75 & 50 & 25 & 10 & 0
% & \textit{Full}$^\dagger$ & 100 & 75 & 50 & 25 & 10 & 0
% & \textit{Full}$^\dagger$ & 100 & 75 & 50 & 25 & 10 & 0 \\
% \midrule
% LongCLIP-FT
% & 64.49 & 62.02 & 59.09 & 48.67 & 35.49 & 28.24 & 0.02
% & 3.20 & 2.97 & 2.96 & 2.47 & 1.73 & 1.63 & 0.03
% & 8.20 & 7.41 & 6.03 & 5.35 & 4.26 & 3.81 & 0.11 \\
% GOAL
% & 79.47 & 66.40 & 63.31 & 53.11 & 39.46 & 31.10 & 0.02
% & 3.52 & 2.90 & 2.85 & 2.45 & 1.82 & 1.84 & 0.03
% & 8.81 & 7.73 & 6.73 & 4.76 & 3.60 & 2.72 & 0.16 \\
% StructXLIP
% & 83.04 & 66.98 & 63.80 & 53.20 & 38.75 & 30.40 & 0.02
% & 3.81 & 3.01 & 2.97 & 2.72 & 1.88 & 2.00 & 0.03
% & 9.93 & 8.00 & 7.30 & 5.93 & 3.90 & 3.28 & 0.16 \\
% \bottomrule
% \end{tabular}%
% }

% \vspace{2pt}
% {\scriptsize $^\dagger$\textit{Full}: original complete caption. 
% $k\in\{100,75,50,25,10,0\}\%$: salient-text keep ratio, with all non-salient text removed.}
% \end{table}
\begin{table}[t]
\centering
\caption{
\textbf{Salient-only diagnosis.}
We feed each model only the top-$k\%$ most salient phrases of every caption, with all non-salient context removed.
Cells report R@1 (\%) on text-to-image retrieval.
The \textit{Full}$^\dagger$ column reports each model's R@1 using the original complete caption.
The bar below each $k$ cell visualizes the recovery ratio R@1$/$\textit{Full}.
The near-random performance at $k{=}0$ serves as a sanity check, since both salient and non-salient text are removed.
}
\label{tab:salient_only}
\scriptsize
\setlength{\tabcolsep}{2.2pt}
\renewcommand{\arraystretch}{1.25}

\newcommand{\rec}[2]{%
  \begin{tabular}[c]{@{}c@{}}
    #2\\[-0.7ex]
    \tikz[baseline=0pt]{%
      \draw[gray!25, line width=0.2pt] (0,0) rectangle (7mm, 0.7mm);
      \fill[recblue!75] (0,0) rectangle (#1*7mm, 0.7mm);
    }
  \end{tabular}%
}

\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}l ccccccc | ccccccc | ccccccc@{}}
\toprule
& \multicolumn{7}{c|}{\textbf{DOCCI}}
& \multicolumn{7}{c|}{\textbf{PathGen}}
& \multicolumn{7}{c}{\textbf{INSECT}} \\
\cmidrule(lr){2-8}\cmidrule(lr){9-15}\cmidrule(lr){16-22}
Model
& \textit{Full}$^\dagger$ & 100 & 75 & 50 & 25 & 10 & 0
& \textit{Full}$^\dagger$ & 100 & 75 & 50 & 25 & 10 & 0
& \textit{Full}$^\dagger$ & 100 & 75 & 50 & 25 & 10 & 0 \\
\midrule
LongCLIP-FT
& 64.49 & \rec{0.96}{62.02} & \rec{0.92}{59.09} & \rec{0.75}{48.67} & \rec{0.55}{35.49} & \rec{0.44}{28.24} & \rec{0.00}{0.02}
& 3.20  & \rec{0.93}{2.97}  & \rec{0.93}{2.96}  & \rec{0.77}{2.47}  & \rec{0.54}{1.73}  & \rec{0.51}{1.63}  & \rec{0.01}{0.03}
& 8.20  & \rec{0.90}{7.41}  & \rec{0.74}{6.03}  & \rec{0.65}{5.35}  & \rec{0.52}{4.26}  & \rec{0.46}{3.81}  & \rec{0.01}{0.11} \\
GOAL
& 79.47 & \rec{0.84}{66.40} & \rec{0.80}{63.31} & \rec{0.67}{53.11} & \rec{0.50}{39.46} & \rec{0.39}{31.10} & \rec{0.00}{0.02}
& 3.52  & \rec{0.82}{2.90}  & \rec{0.81}{2.85}  & \rec{0.70}{2.45}  & \rec{0.52}{1.82}  & \rec{0.52}{1.84}  & \rec{0.01}{0.03}
& 8.81  & \rec{0.88}{7.73}  & \rec{0.76}{6.73}  & \rec{0.54}{4.76}  & \rec{0.41}{3.60}  & \rec{0.31}{2.72}  & \rec{0.02}{0.16} \\
StructXLIP
& 83.04 & \rec{0.81}{66.98} & \rec{0.77}{63.80} & \rec{0.64}{53.20} & \rec{0.47}{38.75} & \rec{0.37}{30.40} & \rec{0.00}{0.02}
& 3.81  & \rec{0.79}{3.01}  & \rec{0.78}{2.97}  & \rec{0.71}{2.72}  & \rec{0.49}{1.88}  & \rec{0.52}{2.00}  & \rec{0.01}{0.03}
& 9.93  & \rec{0.81}{8.00}  & \rec{0.74}{7.30}  & \rec{0.60}{5.93}  & \rec{0.39}{3.90}  & \rec{0.33}{3.28}  & \rec{0.02}{0.16} \\
\bottomrule
\end{tabular}%
}
\vspace{2pt}
{\scriptsize $^\dagger$\textit{Full}: original complete caption. 
$k\in\{100,75,50,25,10,0\}\%$: salient-text keep ratio, with all non-salient text removed. 
Bars below each cell show the recovery ratio R@1$/$\textit{Full}.}
\end{table}

Human users describe salient scene accompanied with contextual part of the scene in the query text. It is likely human users may only provide part of the salient scene in the query text or with mostly context description.
Our preliminary analysis show that sota methods on long-text alignment predominantly align salient text to visual content, leading to fragile alignment when salient text is partially/wholly missing from the retrieval text.

we might need to show: reduced salient text at reduced level (e.g. 100\%, 50\%, 0\%), AND salient text at reduced level  (e.g. 100\%, 50\%, 0\%) + non-salient text. We can use this to show the impact of non-salient text, so this is more relevant to our decomposition idea in the method.

% \input{section/results/preliminary}

==> section/results/supp_differentpair.tex <==
\begin{table}[htbp]
    \centering
    \caption{\textbf{Region selection experiments.} Results on INSECT and DOCCI using different local regions.}
    \label{tab:region_selection} 
    
    \resizebox{\columnwidth}{!}{
        \begin{tabular}{@{}l *{5}{c!{\color{lightlightgray}\vrule width 0.5pt}}c|*{5}{c!{\color{lightlightgray}\vrule width 0.5pt}}c @{}}
        \toprule
        \multirow{2}{*}{\shortstack[c]{\textbf{Methods}}} &
        \multicolumn{6}{c|}{\cellcolor{gray!15}\textbf{INSECT}} &
        \multicolumn{6}{c}{\cellcolor{gray!15}\textbf{DOCCI}} \\
        \cmidrule(lr){2-7}\cmidrule(lr){8-13}
        & \multicolumn{1}{c}{\cellcolor{lightpink}{R@1}} & \multicolumn{1}{c}{\cellcolor{lightpink}{R@5}} & \multicolumn{1}{c}{\cellcolor{lightpink}{R@10}}
        & \multicolumn{1}{c}{\cellcolor{lightblue}{R@1}} & \multicolumn{1}{c}{\cellcolor{lightblue}{R@5}} & \multicolumn{1}{c|}{\cellcolor{lightblue}{R@10}}
        & \multicolumn{1}{c}{\cellcolor{lightpink}{R@1}} & \multicolumn{1}{c}{\cellcolor{lightpink}{R@5}} & \multicolumn{1}{c}{\cellcolor{lightpink}{R@10}}
        & \multicolumn{1}{c}{\cellcolor{lightblue}{R@1}} & \multicolumn{1}{c}{\cellcolor{lightblue}{R@5}} & \multicolumn{1}{c}{\cellcolor{lightblue}{R@10}} \\
        \midrule
        Baseline & 8.81 
 & 24.53 & 35.41  &7.43 & 24.35 & 36.53 & 81.18  &96.67   & 98.51 & 80.00 & 96.31 &98.67 \\
        \midrule
        \rowcolor{gray!8}
        \multicolumn{13}{l}{\textit{Local Region}} \\
        Random Crop & 10.02 & 27.46 & 38.26  & 9.41 & 27.89 & 39.46 & 83.00&	97.45	&99.06	&81.98	&96.71 &	98.76 \\
        \midrule
        \rowcolor{gray!8}
        \multicolumn{13}{l}{\textit{Segmentation-based}} \\
        SAM3 & 8.98  & 26.86 & 38.34  & 8.64 & 26.25 & 37.56 & 82.86&	97.25	&99.08	&81.78&97.10	&98.67 \\
        \midrule
        \rowcolor{gray!8}
        \multicolumn{13}{l}{\textit{Saliency-based}} \\
        % ADMNet & 8.38 & 26.42 & 39.90 & 8.20 & 25.39 & 39.38 & 83.02	&97.63	&99.08	&81.33&	97.18&	98.88 \\
        FASA & \textbf{10.36}
         & \textbf{28.32} & \textbf{40.67} &\textbf{9.84} & \textbf{29.36} & \textbf{40.41} & \textbf{84.35}
         & \textbf{97.51} & \textbf{99.18} &\textbf{82.18} & \textbf{97.14} & \textbf{98.94}  \\
        \bottomrule
        \end{tabular}
    }
\end{table}

==> section/tables/length-controlled.tex <==
\begin{table}[t]
\centering
\caption{
\textbf{Length-controlled analysis under progressive salient reduction.}
Each cell reports the relative R@1 drop under salient deletion / matched random-span deletion, computed with respect to each model's original R@1.
The \textit{removed (\%)} row shows the fraction of caption tokens removed at each $\alpha$.
All numbers are percentages.
A negative random-span drop means that matched random deletion slightly improves R@1.
Across datasets and baselines, deleting salient text causes much larger degradation than deleting random contiguous spans of the same length. \yiming{transform to figures, 2 by 3, two rows for datasets, columen for each method.}
}
\label{tab:preliminary_analysis}

\footnotesize
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.15}

\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}l ccc ccc ccc@{}}
\toprule
& \multicolumn{3}{c}{\textbf{DOCCI}}
& \multicolumn{3}{c}{\textbf{PathGen}}
& \multicolumn{3}{c}{\textbf{INSECT}} \\
\cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}
Model
& $\alpha\!=\!75$ & $\alpha\!=\!25$ & $\alpha\!=\!0$
& $\alpha\!=\!75$ & $\alpha\!=\!25$ & $\alpha\!=\!0$
& $\alpha\!=\!75$ & $\alpha\!=\!25$ & $\alpha\!=\!0$ \\
\textit{removed (\%)}
& \textcolor{mildblue}{5.67} & \textcolor{midorange}{33.70} & \textcolor{severered}{57.95}
& \textcolor{mildblue}{1.96} & \textcolor{midorange}{31.28} & \textcolor{severered}{67.30}
& \textcolor{mildblue}{6.45} & \textcolor{midorange}{34.31} & \textcolor{severered}{65.53} \\
\midrule
LongCLIP-FT
& 11.48/1.78 & 34.07/16.68 & 67.88/39.17
& 58.08/1.97 & 69.00/22.93 & 85.81/57.42
& 49.24/6.28 & 55.84/17.86 & 66.34/24.78 \\
GOAL
& \phantom{0}7.70/1.59 & 26.53/15.74 & 62.50/37.76
& 25.43/1.54 & 56.07/28.52 & 89.60/69.94
& 17.00/1.82 & 34.82/22.47 & 61.94/47.77 \\
StructXLIP
& 10.29/1.53 & 29.39/15.53 & 63.27/37.90
& 33.54/0.84 & 56.18/20.75 & 87.00/63.94
& 21.24/6.43 & 39.42/24.28 & 65.48/50.59 \\
\bottomrule
\end{tabular}%
}
\end{table}
